Impact Invariant Control with Applications to Bipedal Locomotion

When legged robots impact their environment, they undergo large changes in their velocities in a small amount of time. Measuring and applying feedback to these velocities is challenging, and is further complicated due to uncertainty in the impact model and impact timing. This work proposes a general framework for adapting feedback control during impact by projecting the control objectives to a subspace that is invariant to the impact event. The resultant controller is robust to uncertainties in the impact event while maintaining maximum control authority over the impact invariant subspace. We demonstrate the utility of the projection on a walking controller for a planar five-link-biped and on a jumping controller for a compliant 3D bipedal robot, Cassie. The effectiveness of our method is shown to translate well on hardware.

==> chapters/appendices.tex <==
\section{Appendices}


\subsection{Derivation of No-Slip Rigid Body Reset Map}
\label{app:rigid_impact_model}

Using the instantaneous impact assumption and no-slip condition restated below:
\begin{align}
	M(v^+ - v^-) &= J^T \Lambda\\
	Jv^+ = 0
\end{align}
we can solve for the contact impulse $\Lambda$ and post-impact velocity $v^+$.
\begin{align}
	v^+ - v^- &= M^{-1} J^T \Lambda \nonumber\\
	Jv^+ - Jv^- &= J M^{-1} J^T \Lambda \nonumber\\
	\Lambda &= - (J M^{-1} J^T)^{-1} J v^-\\
	v^+ &= v^- - M^{-1} J^T (J M^{-1} J^T)^{-1} J v^- \nonumber\\
	v^+ &= (I - M^{-1} J^T (J M^{-1} J^T)^{-1} J) v^-
\end{align}

\subsection{Mapping Cost-to-go Across Impacts}
\label{app:hlqr_mapping}

Under the instantaneous impact assumption, the cost-to-go cannot change during the impact event, which results in the expression:
\begin{align}
\lim_{t \rightarrow t^-} \tilde{x}(t)^T S(t) \tilde{x}(t) &= \lim_{t \rightarrow t^+} \tilde{x}(t)^T S(t) \tilde{x}(t)
\end{align}
Using (\ref{eq:reset_map}), we can relate $\tilde{x}^-$ and $\tilde{x}^+$ with the linearized reset map $\hat{R}$:
\begin{align}
\lim_{t \rightarrow t^-} \tilde{x}(t) = \hat{R} \lim_{t \rightarrow t^+} \tilde{x}(t)
\end{align}
Through substitution, we arrive at the expression to map $S$ across an impact event.
\begin{align}
S(t^-) &= \hat{R}^T S(t^+) \hat{R}
\end{align}

\subsection{Finding Gaits using Trajectory Optimization}
\label{app:traj_opt}

The walking and jumping gaits were found through trajectory optimization by formulating them as constrained direct collocation problems and solving using a C++ implementation of DIRCON \cite{posa2016optimization}.
For both trajectories, I imposed no-slip contact constraints on the feet that were defined to be in stance as well as appropriate joint and actuator limits.
These can both be represented as the following optimization problem:
\begin{align}
	\min_{x_k, u_k}   &\quad&  \sum_{k} g(x_k, u_k) + g_f(x_N) &&  & \\
	\text{subject to: } 
	&\quad&  c(x, u) = 0 &&  & \\
	&\quad&  \phi(q) = \psi(x) = \alpha(x, u, \lambda) = 0 \\
	&\quad&  h(x, u) \geq 0  &&  &
\end{align}
\noindent where $g$ is a cost on the states and inputs, typically defined to be the $u^T u$ plus some normalization terms.
$c$ are the equality constraints such as the dynamics constraints at the collocation points and $h$ are the inequality constraints such as joint and actuator limits.
$\phi$ and its first and second time derivatives $\psi$ and $\alpha$ respectively are kinematic constraints.
These are the no-slip contact constraints and for Cassie specifically, the loop closure constraint between the thigh and the hip.

The walking trajectory was composed of two modes, with a single foot in stance per mode.
I set periodic constraints, which enforced that the final state must equal the initial state except for the global x position of the hip, which was instead constrained to translate 0.3m over the full trajectory.
I also set symmetry constraints between the left and right legs; note that setting symmetry constraints is equivalent to generating a trajectory for a single stance mode and simply mirroring the state to construct the trajectory for the second mode.
I chose to set symmetry constraints for the ease of not having to post-process the final trajectory.

The jumping trajectory consisted of three modes {CROUCH, FLIGHT, STANCE}.
All four points of contact of Cassie were constrained to be on the ground for both the CROUCH and STANCE modes.
To enforce a jumping motion, I set that the height of the pelvis must be 0.2 m above the initial starting height, which was set at 1.075m.
I also constrained the initial and final state to have zero initial velocity to prevent the optimizer from abusing initial kinematic energy in the system.

==> chapters/results.tex <==
\section{Results}
\label{sec:results}


\subsection{Simulation Results of the OSC Jumping Controller}
	
	\begin{figure}
		\centering
		\includegraphics[width=0.48\textwidth]{figures/param_study_power_loss_height.png}
		\includegraphics[width=0.48\textwidth]{figures/param_study_accel_err_height.png}
		\caption{Results from the parameter sweep over unexpected landing heights. The controllers with the impact invariant projection has significantly less power losses (top) compared to the default controller across all terrain heights. The projection also reduces the weighted acceleration error (bottom), though the benefit is sensitive to the duration of the projection.}
		\label{fig:param_study_results}
	\end{figure}
	
	We evaluate the controller performance based on two metrics, the control effort and the acceleration error at the end of the impact event.
	
	\subsubsection{Control Effort}
	We quantify the control effort used to stabilize the robot upon landing using the objective
	\begin{align*}
		J_{mot} = \int_{0}^{T} u^2 dt.
	\end{align*}
	We choose this as a measure for how hard the actuators are working, with the idea that minimal control effort is desirable especially when applying feedback control when the state is so uncertain.
	\subsubsection{Acceleration Error}
	We used the weighted acceleration error in the output space to measure the tracking error after impact.
	This is also the feedback terms in from \eqref{eq:output_cmd} repeated here:
	\begin{align*}
		\ddot y_{err} &= K_p (y_{des} - y) - K_d (\dot{y}_{des} - \dot y)\\
		J_{acc} &= \sum_{i = 0}^{N} \ddot y_{i, err}^T W_i \ddot y_{i, err}
	\end{align*}
	We choose this as a way to combine position and velocity error into a single metric.
	We evaluate the acceleration error in a window at end of the longest projection window because after this point, all the controllers are identical.
	To avoid bias from sampling at a particular time step, we sample multiple points near the desired sample time.
	To put the acceleration error in context, we normalize the acceleration error so that an acceleration error of 1 corresponds to a tracking error of 7cm for the vertical position of the pelvis.
	
	The results from the sweep over changes in the landing platform height is shown in \ref{fig:param_study_results}.
	We did not observe a significant amount of sensitivity to changes in the ground stiffness.

%		\begin{table}[ht]
%			\centering
%			\caption{Tracking performance improvement}
%			\begin{tabular}{c||c|c}
%				duration & peak actuator effort & CoM accel error (med, stdev) \\
%				\hline
%				0ms & 130Nm & 2.77, 0.22\\
%				25ms & 89Nm & 2.28, 0.08 \\ 
%				50ms & 89Nm & 2.30, 0.06 \\ 
%				75ms & 112Nm & 1.06, 0.66 \\ 
%				100ms & 91Nm & 1.80, 0.16
%			\end{tabular}
%		\end{table}
		

	
%	\subsubsection{MUJOCO simulator}
%	\subsubsection{Five Link Biped Walking Controller}
%		We develop three versions of a joint-space OSC as a point of comparison. 
%		The first controller is a conventional OSC
%	
%		\begin{figure}
%			\centering
%			\includegraphics[width=0.45\textwidth]{figures/swing_leg_velocity_error.png}
%			\includegraphics[width=0.45\textwidth]{figures/stance_leg_velocity_error.png}
%			\caption{The joint velocity error in the impact sensitive leg is given in the top figure and the other leg which should maintain most of the velocity tracking is given in the bottom figure. The directional robustness of the impact invariant projection is clearly shown here: the impact invariant feedback controller does not introduce error during the impact event while still maintaining more control of the other states. This essentially give it the best of both worlds.}
%			\label{fig:directional_robustness}
%		\end{figure}
		
	
\subsection{Experimental Results}
	
%	The operational space version of the jumping controller was implemented on the Cassie hardware using the same reference trajectory.
%	The sensing was limited to onboard joint encoders and IMU.
%	Due to model differences and state uncertainty from the state estimator and noisy encoder data, the tracking performance of the controller was less good on hardware.
%	A fixed time offset of 75ms was added to the nominal landing time of the time-based finite state machine to coincide closer with the actual impact time.
	
	Experiments using the controller with and without the impact invariant projection were both consistently able to successfully complete the jump.
	The peak motor efforts especially at the start of the landing phase are significantly reduced when using the impact invariant projection as seen in Figure \ref{fig:hardware_knee_efforts}.
	The smoothing out of the commanded motor efforts is similar to what we see in simulation.
%	 - the projection effectively smooths out the commanded actuator efforts around the impact time.
		
	\begin{figure}
		\centering
		\includegraphics[width=0.48\textwidth]{figures/jan_27_hardware_knee_efforts.png}
		\caption{Motor efforts on Cassie executing the jumping motion. The combined knee motor torques commanded by the jumping controller are shown for three different durations of the impact invariant projection.}
		\label{fig:hardware_knee_efforts}
	\end{figure}
	

	
